LLMs for Generating and Evaluating Counterfactuals: A Comprehensive Study

As NLP models become more complex, understanding their decisions becomes more crucial. Counterfactuals (CFs), where minimal changes to inputs flip a model's prediction, offer a way to explain these models. While Large Language Models (LLMs) have shown remarkable performance in NLP tasks, their efficacy in generating high-quality CFs remains uncertain. This work fills this gap by investigating how well LLMs generate CFs for two NLU tasks. We conduct a comprehensive comparison of several common LLMs, and evaluate their CFs, assessing both intrinsic metrics, and the impact of these CFs on data augmentation. Moreover, we analyze differences between human and LLM-generated CFs, providing insights for future research directions. Our results show that LLMs generate fluent CFs, but struggle to keep the induced changes minimal. Generating CFs for Sentiment Analysis (SA) is less challenging than NLI where LLMs show weaknesses in generating CFs that flip the original label. This also reflects on the data augmentation performance, where we observe a large gap between augmenting with human and LLMs CFs. Furthermore, we evaluate LLMs' ability to assess CFs in a mislabelled data setting, and show that they have a strong bias towards agreeing with the provided labels. GPT4 is more robust against this bias and its scores correlate well with automatic metrics. Our findings reveal several limitations and point to potential future work directions.

==> src/analysis.tex <==
%Our results so far show that SA CFs have high quality (cf. Table~\ref{tab:robustness} and~\ref{tab:sent:augmentation}), whereas the results for NLI CFs are less encouraging (cf. Table~\ref{tab:robustness} and~\ref{tab:nli:augmentation}).

Our evaluation so far includes intrinsic properties to assess the quality of the obtained CFs (Section~\ref{eval:intrinsic}), and estimating the utility of CFs for detecting and addressing model failures (Section~\ref{eval:robustness} and ~\ref{eval:augmentation}). Since recent work shows that evaluating with LLMs is often consistent with human evaluation~\cite{chiang-lee-2023-large}, we conduct an LLM evaluation with GPT3.5. Our goal is to examine CFs in more depth. Our evaluation focuses on the three aspect that are deemed most important in CFs: 
\begin{itemize}
    \item Label flipping: Does the generated CF really have the target label?
    \item Minimal changes: Are there any unnecessary changes in the CF?
    \item Feature Distribution Alignment: Is the CF realistic?
\end{itemize}

We ask GPT3.5 to evaluate human and LLMs CFs with respect to the aforementioned aspects. For each question, a score between 1 and 4 should be selected (higher is better). The exact prompt can be found in \ref{} in Appendix~\ref{}.  ~\ref{fig:large-text}

\begin{table}[]
    \centering
\begin{tabular}{lrrr}
%\begin{tabularx}{\columnwidth}{p^{2cm}p^{2cm}p^{3cm}p^{2cm}}
\toprule
        LLM &  FL &  Min. &  Dist.  \\
\midrule
      crowd &               3.43 &                     2.78 &                 2.94 \\
     expert &               3.35 &                     2.74 &                 2.93 \\
     gpt3.5 &               3.28 &                     2.82 &                 2.96 \\
       gpt4 &               3.55 &                     2.90 &                 3.06 \\
     llama2 &               3.30 &                     2.82 &                 2.97 \\
 llama2\_70b &               3.41 &                     2.85 &                 2.98 \\
    mistral &               3.48 &                     2.83 &                 2.97 \\
mistral\_56b &               3.00 &                     2.62 &                 2.74 \\
\bottomrule
\end{tabular}
%\end{tabularx}

    \caption{Caption}
    \label{tab:my_label}
\end{table}




==> src/app_data.tex <==
Some statistics about the number of generated CFs are shown in Table~\ref{tab:data_stats}.

\begin{table}[]
    \centering
    \footnotesize
\begin{tabular}{lllr}
\toprule
     task &                                     llm &            split &  size \\
\midrule
      nli &                  NLI\_revised\_hypothesis &              dev &   400 \\
      nli &                  NLI\_revised\_hypothesis &             test &   800 \\
      nli &                  NLI\_revised\_hypothesis &            train &  3332 \\
      nli &                     NLI\_revised\_premise &              dev &   400 \\
      nli &                     NLI\_revised\_premise &             test &   800 \\
      nli &                     NLI\_revised\_premise &            train &  3332 \\
      nli &      gpt3.5\_revised\_hypothesis &              dev &   400 \\
      nli &      gpt3.5\_revised\_hypothesis &             test &   800 \\
      nli &      gpt3.5\_revised\_hypothesis &            train &  3332 \\
      nli &         gpt3.5\_revised\_premise &              dev &   400 \\
      nli &         gpt3.5\_revised\_premise &             test &   800 \\
      nli &         gpt3.5\_revised\_premise &            train &  3330 \\
      nli &        gpt4\_revised\_hypothesis &              dev &   400 \\
      nli &        gpt4\_revised\_hypothesis &             test &   800 \\
      nli &        gpt4\_revised\_hypothesis &            train &  3329 \\
      nli &           gpt4\_revised\_premise &              dev &   400 \\
      nli &           gpt4\_revised\_premise &             test &   800 \\
      nli &           gpt4\_revised\_premise &            train &  3332 \\
      nli &      llama2-7b\_revised\_hypothesis &              dev &   335 \\
      nli &      llama2-7b\_revised\_hypothesis &             test &   797 \\
      nli &      llama2-7b\_revised\_hypothesis &            train &  3312 \\
      nli &         llama2-7b\_revised\_premise &              dev &   280 \\
      nli &         llama2-7b\_revised\_premise &             test &   768 \\
      nli &         llama2-7b\_revised\_premise &            train &  3198 \\
      nli &  llama2\_70b\_revised\_hypothesis &              dev &   116 \\
      nli &  llama2\_70b\_revised\_hypothesis &             test &   174 \\
      nli &  llama2\_70b\_revised\_hypothesis &            train &   582 \\
      nli &     llama2\_70b\_revised\_premise &              dev &    84 \\
      nli &     llama2\_70b\_revised\_premise &             test &   122 \\
      nli &     llama2\_70b\_revised\_premise &            train &   481 \\
      nli &     mistral-7b\_revised\_hypothesis &              dev &   380 \\
      nli &     mistral-7b\_revised\_hypothesis &             test &   755 \\
      nli &     mistral-7b\_revised\_hypothesis &            train &  3150 \\
      nli &        mistral-7b\_revised\_premise &              dev &   379 \\
      nli &        mistral-7b\_revised\_premise &             test &   769 \\
      nli &        mistral-7b\_revised\_premise &            train &  3174 \\
      nli & mistral\_56b\_revised\_hypothesis &              dev &   257 \\
      nli & mistral\_56b\_revised\_hypothesis &             test &   516 \\
      nli & mistral\_56b\_revised\_hypothesis &            train &  2076 \\
      nli &    mistral\_56b\_revised\_premise &              dev &   270 \\
      nli &    mistral\_56b\_revised\_premise &             test &   518 \\
      nli &    mistral\_56b\_revised\_premise &            train &  2126 \\

      sentiment &                           experts &              dev &   245 \\
sentiment &                           experts &             test &   488 \\

sentiment &                           crowd &              dev &   245 \\
sentiment &                           crowd &             test &   488 \\
sentiment &                           crowd &            train &  1707 \\
sentiment &                     gpt3.5 new &              dev &   245 \\
sentiment &                     gpt3.5 new &             test &   488 \\
sentiment &                     gpt3.5 new &            train &  1707 \\
sentiment &                       gpt4 new &              dev &   245 \\
sentiment &                       gpt4 new &             test &   486 \\
sentiment &                       gpt4 new &            train &  1704 \\
sentiment &                     llama2-7b new &              dev &   243 \\
sentiment &                     llama2-7b new &             test &   483 \\
sentiment &                     llama2-7b new &            train &  1681 \\
sentiment &                 llama2\_70b new &              dev &    88 \\
sentiment &                 llama2\_70b new &             test &   325 \\
sentiment &                 llama2\_70b new &            train &   738 \\
sentiment &                    mistral-7b new &              dev &   200 \\
sentiment &                    mistral-7b new &             test &   411 \\
sentiment &                    mistral-7b new &            train &  1439 \\
sentiment &                mistral\_56b new &              dev &   150 \\
sentiment &                mistral\_56b new &             test &   275 \\
sentiment &                mistral\_56b new &            train &  1026 \\
\bottomrule
\end{tabular}
    \caption{Statistics of datasets used and generated}
    \label{tab:data_stats}
\end{table}

==> src/app_human_corr.tex <==
We also compare GPT4 annotations to human annotations on a sample of 28 instances. More specifically, we choose 4 NLI CFs for each LLM, along with 4 examples from human CFs. Two of the authors independently annotated this sample using the same instructions given to GPT4, and then resolved any discrepancies. The flip label scores distribution based on the authors' and GPT4 annotations can be shown in Table~\ref{tab:flip_label_dist_humans}. We end up with 27 examples, since GPT4 refused to annotate one CF for being ``too short''. The Spearman correlation between the agreed-upon annotations and the annotations from GPT4 is 0.69 (strong correlation). Based on this positive outcome, 

% Move to appendix ?
\begin{table}[]
    \centering
        \begin{tabular}{ccc}
        \toprule
        \textbf{Score}  & \textbf{Human}   & \textbf{GPT-4}\\
        \midrule
        1 &            35.71    & 29.62 \\
        2 &            14.29   & 3.70 \\
        3 &            14.29   & 3.70\\
        4 &            35.71   & 62.97\\
        
        \bottomrule
        \end{tabular}
    \caption{Distributions of flip label scores on sample of 28 examples from human and GPT-4 annotations.}
    \label{tab:flip_label_dist_humans}
\end{table}

==> src/draft_py.tex <==
\begin{table}[]
    \centering
\begin{tabularx}{\columnwidth}{p{6cm}p{1cm}}
\toprule
       \textbf{Training Data} &  \textbf{Acc.} \\
\midrule

     \textbf{crowd Both} & \\

 \midrule
  crowd orig &     49.19 \\ 
 crowd all\_combined &     68.31 \\\midrule 
     gpt3.5 all\_combined &     53.75 \\
       gpt4 all\_combined &     57.25 \\
         llama2 7b all\_combined &     53.69 \\
 llama2 70b all\_combined &     55.81 \\
 mistral 7b all\_combined &     50.62 \\ 
mistral 56b all\_combined &     41.75 \\\midrule 
     \textbf{crowd Hypothesis} & \\

 \midrule
  crowd orig &     58.50 \\ 
      crowd all\_combined &     71.25 \\ \midrule 
     gpt3.5 all\_combined &     51.88 \\
       gpt4 all\_combined &     58.63 \\
  llama2 7b all\_combined &     51.12 \\
   llama2 70b all\_combined &     58.13 \\

   mistral 7b all\_combined &     48.38 \\
mistral 56b all\_combined &     39.75 \\
 \midrule 
     \textbf{crowd Premise} & \\

 \midrule
 crowd orig &     39.88 \\
      crowd all\_combined &     65.38 \\ \midrule 
     gpt3.5 all\_combined &     55.62 \\
       gpt4 all\_combined &     55.88 \\
  llama2 7b all\_combined &     56.25 \\
 llama2 70b all\_combined &     53.50 \\
 mistral 7b all\_combined &     52.88 \\ 
mistral 56b all\_combined &     43.75 \\\midrule 
     \textbf{original} & \\

 \midrule
 
              crowd orig &     73.50 \\ 
              crowd all\_combined &     78.50 \\\midrule 
     gpt3.5 all\_combined &     55.00 \\ 
       gpt4 all\_combined &     70.75 \\
 llama2 70b all\_combined &     65.75 \\
  llama2 7b all\_combined &     57.50 \\
 mistral 7b all\_combined &     57.75 \\
 mistral 56b all\_combined &     45.75 \\

\bottomrule

 
\end{tabularx}

    \caption{Data augmentation results for SA. Classification model is trained on original and LLMs or human-generated CFs.}
    \label{tab:nli:augmentation}
\end{table}

==> src/examples/nli_hypo.tex <==

\begin{table*}
\tiny
\begin{tabular}{lp{2cm}p{2cm}p{2cm}llrrr}
\toprule
        LLM &      Premise &  F Hypothesis &  CF Hypothesis & original label & target label &  flip\_label &  Min. &  Dist. \\
\midrule
       gpt4 &                                                                                                                                          A little girl drawing with chalk, on a chalkboard. &                A little girl is drawing on the board during class. &                                                                     A little boy is not drawing on the chalkboard not during class. &        neutral &  contradiction &         1.0 &               1.0 &           2.0 \\
       gpt4 &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &                                                                            The photographer is taking a photo of a man and a woman. &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
      crowd &                                                                                                                         An old man in a blue shirt and white pants glowers by a glass door. &                                              A man resting outside &                                                                                                              A glass man by a door. &        neutral &  contradiction &         1.0 &               1.0 &           1.0 \\
      crowd &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &                                                                            The photographer is taking a photo of a man and a woman. &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
    mistral &                                                           A man in a black shirt and brown pants is jumping in the air performing a karate kick towards a man in a red shirt and black hat. &                            Two males are involved in martial arts. & A woman in a red dress and blue scarf is standing still facing each other. The female model wearing sunglasses is playing football. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
    mistral &                                                                                                         At least eight people are sitting at a table in a building that overlooks the city. &                                        People sitting on the floor &                                    At least eight people are sitting at a table on the floor in a building that overlooks the city. &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
mistral\_56b &                                                                                A man with a beard is talking on the cellphone and standing next to someone who is lying down on the street. & A man is prone on the street while another man stands next to him. &                                                                              Unproning on the street while another man lies in bed. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
mistral\_56b &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &                                                                                     The photographer is taking a photo of anything. &  contradiction &        neutral &         4.0 &               4.0 &           4.0 \\
     gpt3.5 &                                                                                                                                          Two people are participating in the sport fencing. &                       Two people competing in a fencing tournament &                                                                                                   The statement is a contradiction. &        neutral &     entailment &         1.0 &               1.0 &           1.0 \\
     gpt3.5 &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &     The photographer is taking a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
 llama2\_70b &                                                                                     A boy dressed for summer in a green shirt and kahki shorts extends food to a reindeer in a petting zoo. &   A boy alien dressed for summer in a green shirt and kahki shorts &                                                                   A girl alien dressed for summer in a green shirt and kahki shorts &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
 llama2\_70b &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &                                                  The photographer takes a photo of a dog and a man in a suit and a woman in a dress &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
     llama2 & An Asian woman in a purple shirt preparing a bowl of food for the younger Asian boy sitting near buy, while an Asian man eats a roll and prepares to take some food up with his chopsticks. &                             A woman is preparing food for a child. &                                                                        A Caucasian woman is not preparing food for a Caucasian boy. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
     llama2 &                                                      A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                       The photographer is taking a photo of a dog. &                                                  a man in a suit and a woman in a dress stand in front of columns and a yellow wall &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
\bottomrule
\end{tabular}

    \caption{NLI - revised hypothesis examples}
    \label{tab:examples:hypothesis}
    
\end{table*}

==> src/examples/nli_premise.tex <==
\begin{table*}[]
    \centering
    \tiny
\begin{tabular}{lp{2cm}p{2cm}p{2cm}llrrr}
\toprule
        LLM &   F Premise &  CF Premise &                                               Hypothesis  & original label & target label &  flip\_label &  Min. &  Dist \\
\midrule
       gpt4 &                                                                                 An older man sifts water through his fingers as a young toddler watches from inside the water. &                                                                                         An older man sifts water through his fingers as a young toddler is far from any toddler. &                                          A man is near a toddler &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
       gpt4 &                                         A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                                                                                                                                     The photographer is taking a photo of a dog. &                     The photographer is taking a photo of a dog. &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\ 
      crowd & In an apparent classroom setting, a young man in a blue t-shirt has a book on his knee while a woman dressed in black next to him leans in to point out something in the book. & In an apparent classroom setting, a young woman in a blue t-shirt has a book on his knee while a woman dressed in black next to him leans in to point out something in the book. &                               The man and woman are cooperating. &        neutral &  contradiction &         1.0 &               1.0 &           1.0 \\
      crowd &                                         A photographer and assistant take a photo of a man in a suit and a woman in a dress in front of large white columns and a yellow wall. &                                                  A photographer and assistant take a photo of a married couple and their pets in front of large white columns and a yellow wall. &                     The photographer is taking a photo of a dog. &  contradiction &        neutral &         4.0 &               4.0 &           4.0 \\
    mistral &                                                                                                                                   Artist on street corner selling his artwork. &                                                                                   Buyer is not on street inside a building and is not far away from somebody else's not artwork. &                                    Someone is selling paintings. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
    mistral &                                                                                            At least eight people are sitting at a table in a building that overlooks the city. &                                                          At least eight people are sitting at a table in a building that overlooks the city. People can be sitting on the floor. &                                      People sitting on the floor &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
mistral\_56b &                                                                                                                    A solo shot of a man riding a four wheeler in an atv event. &                                                                               A solo shot of a man rode a four wheeler in an no atv event. The man is not entered in a no event. &                                   The man is entered in a event. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
mistral\_56b &                                                      People are on an escalator waiting to get to their destination while looking outside of the glass that makes up the wall. &                                                          People are on a elevator waiting to get to their destination while looking outside of the glass that makes up the wall. &                                  People are taking the elevator. &  contradiction &        neutral &         4.0 &               4.0 &           4.0 \\
     gpt3.5 &                                                                        A boy dressed for summer in a green shirt and kahki shorts extends food to a reindeer in a petting zoo. &                                                                                    A boy dressed for summer in a green shirt and khaki shorts does not have food for a reindeer. & A boy alien dressed for summer in a green shirt and kahki shorts &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
     gpt3.5 &                                                      People are on an escalator waiting to get to their destination while looking outside of the glass that makes up the wall. &                                                                                                People are inside a building looking outside of the glass that makes up the wall. &                                  People are taking the elevator. &  contradiction &        neutral &         4.0 &               4.0 &           4.0 \\
 llama2\_70b &                                                                        A boy dressed for summer in a green shirt and kahki shorts extends food to a reindeer in a petting zoo. &                                                                            A girl dressed for winter in a red shirt and black shorts withdraws water from a shark in an aquarium & A boy alien dressed for summer in a green shirt and kahki shorts &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
 llama2\_70b &                                                                                                                              A man in colorful shorts is surfing under a wave. &                                                                                                            A man in colorful shorts is lying beside a wave. A man is sunbathing. &                                             A man is sunbathing. &  contradiction &        neutral &         4.0 &               4.0 &           4.0 \\
     llama2 &                                                                                                                                             A man in a boom lift bucket welds. &                                                                                                                                                    A man in a spoon is painting. &                                                A man is working. &     entailment &  contradiction &         1.0 &               1.0 &           1.0 \\
     llama2 &                                                                                            At least eight people are sitting at a table in a building that overlooks the city. &                                                                                                                                                     People sitting on the floor. &                                      People sitting on the floor &  contradiction &     entailment &         4.0 &               4.0 &           4.0 \\
\bottomrule

\end{tabular}

    \caption{NLI - revised premise examples}
    \label{tab:examples:premise}
\end{table*}

==> src/examples/sent.tex <==
\begin{table*}[]
\tiny
\begin{tabular}{lp{5cm}lp{5cm}lrrr}
\toprule
        LLM &  F &  label &  CF & target label &  FL &  Min &  Dist \\
\midrule
      crowd &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           Greenaway seems to have a habit of trying deliberately to disgust his viewers. This film opens with incest--and purposeless, meaningless, casual incest at that. That's Greenaway's big problem. He prefers parlor tricks to shock over actually doing anything meaningful. Technical skill isn't enough. He's just a bit perverse for the sake of perversity. &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     Greenaway seems to have a habit of trying hard to entertain his viewers. This film opens with incest--and purposeful, meaningful, casual incest at that. That's Greenaway's focus. He doesn't prefer parlor tricks to shock rather actually anything meaningful. Technical skill isn't enough. He's a bit perverse for the sake of perversity but it works out well. &       Positive &         1.0 &               1.0 &           1.0 \\
      crowd &                                                                                                                                                                                                                                                                                                   The most important thing about this movie is the brilliant performance by Daniel Day-Lewis and Hugh O'Conor as Christy Brown, guineas artist and fighter who despite of her physical condition overcame all the odds. As a person who did work with patients with cerebral palsy, I can assure you that their performance were shockingly convincing. The enormous support that Christy got form his family, low-income, working class Dubliners, encouraged him to do the impossible and this picture depicted this support brilliantly have not read the book, but the dialogs were written wisely to capture Christy Brown's witty arrogant personality. I do recommend this movie to everyone, especially to classic movie-lovers. &       Positive &                                                                                                                                                                                                                                                                                    The most annoying thing about this movie is the lackluster performance by Daniel Day-Lewis and Hugh O'Conor as Christy Brown, guineas artist and fighter who despite her physical condition overcame all the odds. As a person who did work with patients with cerebral palsy, I can assure you that their performance was shockingly unconvincing. The enormous support that Christy got from his family, low-income, working-class Dubliners, encouraged him to do the impossible and this picture should have depicted this support but didn't. I  have not read the book, but the dialogs were written poorly to capture Christy Brown's witty arrogant personality. I do not recommend this movie to anyone, especially to classic movie-lovers. &       Negative &         4.0 &               4.0 &           4.0 \\
     expert & Dave is going through a divorce and his mind wanders back to his first love. "Wanders" is probably not the word. I should say he fixates on the past girlfriend. He recalls to the day when the relationship ended. The dream sequences only lack the hazy transitions. He fondly recalls their favorite songs and places they went. I'm not a counselor, but maybe this had something to do with the failed marriage???? Dave goes to a support group and meets up with a lady half his age (also divorced) who, instead of being "turned off" by his creepiness, starts to become interested in him. Did I mention how creepy Dave is? He sometimes refers to himself in the third person. He doesn't move his arms when he walks, either. It's just weird. Too make a long story short, Dave plots to hunt down Mary (the old gal friend) and kill her...err...I mean confront her. He does so. Which was really creepy. He believes her to be married, yet he STILL flies half-way across the country to meet her. He stakes out ... &       Negative & Dave is going through a divorce and his mind wanders back to his first love. "Wanders" is probably not the word. I should say he fixates on the past girlfriend. He recalls to the day when the relationship ended. The dream sequences only lack the hazy transitions. He fondly recalls their favorite songs and places they went. I'm not a counselor, but maybe this had something to do with the failed marriage???? Dave goes to a support group and meets up with a lady half his age (also divorced) who, instead of being "turned off" by his creepiness, starts to become interested in him. Did I mention how creepily good Dave is? He sometimes refers to himself in the third person. He doesn't move his arms when he walks, either. It's just great. Too make a long story short, Dave plots to hunt down Mary (the old gal friend) and kill her...err...I mean confront her. He does so. Which was really funny. He believes her to be married, yet he STILL flies half-way across the country to meet her. He stake... &       Positive &         1.0 &               1.0 &           1.0 \\
     expert & Takashi Miike's incursion into kiddie territory won me over almost immediately because he demonstrates nerve and bravery in dealing with fantasy elements. This is a fairy tale that dares to be dark. Even as a kid, I thought that there was something sinister about most fairy tales; horrible things happen to people in most children's books. Miike understands that these classic tales are a bit scarier (and more disturbing) than what they appear to be at first glance. The filmmaker takes the archetypical story of a kid on a wondrous quest out of the preschool classroom. He accentuates the very real fears of a world filled with never-ending hazardous missions. Westerners like to downplay the seriousness behind bedtime stories written specifically for kids. I appreciated the fact that Miike was more honest than most American filmmakers. He goes for the jugular of the story but he also shows signs of restrain. But a self-possessed Miike is still stranger than most filmmakers. I thought it ... &       Positive & Takashi Miike's incursion into kiddie territory lost me over almost immediately because he demonstrates nerve and bravery in dealing with fantasy elements. This is a fairy tale that dares to be dark. Even as a kid, I thought that there was something sinister about most fairy tales; horrible things happen to people in most children's books. Miike understands that these classic tales are a bit scarier (and more disturbing) than what they appear to be at first glance. The filmmaker takes the archetypical story of a kid on a wondrous quest out of the preschool classroom. He accentuates the very real fears of a world filled with never-ending hazardous missions. Westerners like to downplay the seriousness behind bedtime stories written specifically for kids. I appreciated the fact that Miike was more honest than most American filmmakers. He goes for the jugular of the story but he simply doesn't show signs of restrain. A self-possessed Miike is still stranger than most filmmakers. I didn'... &       Negative &         4.0 &               4.0 &           3.0 \\
     gpt3.5 &                                                                                                                                                                                                                                                                                                                                                                                                                                                          My Favorite part was when the credits started to roll. I wish I could give it a .0000000000001 out of 10. I really wish I had that Hour and thirty minutes back. Don't waste your money or time on it. I really could have watched grass grow and felt better after wards.<br /><br />Nadia was really pretty and I hope the movie didn't destroy her career. But she chose to be in it.<br /><br />All in all it sucked more than any other movie has sucked. More than Kazaam and Glitter combined. That's saying something.<br /><br />Don't<br /><br />Do<br /><br />it!!!! &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                              My Best part was when the credits started to roll. I hope I could give it a 10 out of 10. I really hope I had that Hour and thirty minutes back. Worth watching your money or time on it. I should have watched a beautiful garden bloom and felt even more inspired after wards.<br /><br />Nadia looked stunning and I hope the movie didn't boost her career. But she chose to be in it.<br /><br />All in all it's better than any other movie. More than Kazaam and Glitter combined. That's impressive.<br /><br />Definitely<br /><br />Watch it!!!! &       Positive &         1.0 &               1.0 &           1.0 \\
     gpt3.5 & I was 5 years old when I saw this musical movie while on vacation with my family in St. Thomas in 1977 and immediately fell in love with it. 27 years later, it is still an original inspiration for achieveing my goals that I have set to accomplish since that time!<br /><br />This tragic story of a hard-core "behind the scenes" of the entertainment industry during the late 50's, "Sparkle" successfully portrays the struggle of three young sisters looking for their place in the sun. This story could simply become the biographical story of many young aspiring artists about what could materialize when things seem to happen too fast and role models are not available to lend a helping hand.<br /><br />The phenomenal music written and composed by Aretha Franklin and Curtis Mayfield, the soundtrack carries the plot with every song. From being subjected to situations that almost leave no choice for strong long-term decision-making, to making the ultimate sacrifice in order to get ahead, all th... &       Positive & I was 5 years old when I saw this musical movie while on vacation with my family in St. Thomas in 1977 and immediately fell in love with it. 27 years later, it is still an original inspiration for achieveing my goals that I have set to accomplish since that time!<br /><br />This tragic story of a hard-core "behind the scenes" of the entertainment industry during the late 50's, "Sparkle" successfully portrays the struggle of three young sisters looking for their place in the sun. This story could simply become the biographical story of many young aspiring artists about what could materialize when things seem to happen too fast and role models are not available to lend a helping hand.<br /><br />The lackluster music written and composed by Aretha Franklin and Curtis Mayfield, the soundtrack carries the plot with every song. From being subjected to situations that almost leave no choice for strong long-term decision-making, to making the ultimate sacrifice in order to get ahead, all th... &       Negative &         4.0 &               4.0 &           3.0 \\
       gpt4 &                                                                                                                                                                                                                                                                                                                                                                                                                                      A female country singer nicknamed "Big T"--seriously, that's what they call her--risks her budding musical career and her life by falling into the company of a sleazy drunkard (Busey) who wants to be her manager. His mother committed suicide, his father's an alcoholic as well, and he has a violent temper. You can imagine where that leads. In the meantime, there's music aplenty, as Parton, with her fluid vocal talents, belts out song after song (at least half a dozen of them about Texas). Steer clear of this mess and check her out in NINE TO FIVE or STEEL MAGNOLIAS instead. &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             ', 'risks her budding musical career and her life by', 'sleazy', 'drunkard', 'committed suicide,', 'alcoholic', 'violent temper.', 'You can imagine where that leads.', 'Steer clear of this mess and'\textbackslash n\textbackslash nStep 2: Change these phrases, words, sentences to Positive sentiment with minimal changes: \textbackslash n'Posi &       Positive &         1.0 &               1.0 &           1.0 \\
       gpt4 &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       This movie is really not all that bad. But then again, this movie genre is right down my alley. Sure, the sets are cheap, but they really did decent with what they had. <br /><br />If you like cheap, futuristic, post-apocalyptic B movies, then you'll love this one!! I sure did!<br /><br /> &       Positive &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           This movie is really quite bad. And then again, this movie genre is not my cup of tea. Sure, the sets are cheap, and they failed to convince with what they had. <br /><br />If you like cheap, futuristic, post-apocalyptic B movies, then you'll probably dislike this one!! I certainly didn't.<br /><br /> &       Negative &         4.0 &               4.0 &           4.0 \\
     llama2 &                                                                                                                                                                                                                                                                                                                                                                                                                                      A female country singer nicknamed "Big T"--seriously, that's what they call her--risks her budding musical career and her life by falling into the company of a sleazy drunkard (Busey) who wants to be her manager. His mother committed suicide, his father's an alcoholic as well, and he has a violent temper. You can imagine where that leads. In the meantime, there's music aplenty, as Parton, with her fluid vocal talents, belts out song after song (at least half a dozen of them about Texas). Steer clear of this mess and check her out in NINE TO FIVE or STEEL MAGNOLIAS instead. &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         Joining forces with a seasoned manager, a female country singer nicknamed "Big T" risks her budding musical career and her life. His mother passed away, his father's struggling with addiction, and he has a quick to anger temper. You can imagine where this journey takes us. In the meantime, there's music aplenty, as Parton, with her fluid vocal talents, belts out song after song (at least half a dozen of them about Texas). Steer clear of this mess and check her out in NINE TO FIVE or STEEL MAGNOLIAS instead. &       Positive &         1.0 &               3.0 &           2.0 \\
     llama2 &                                                                                                                                                                                                                                                                                                                                                                              Yeah, the archetype of a simple but inspirational movie. The very end when the entire crowd in the stadium gets up and the people raise their hands gives me a chill whenever I see it. That's just brilliant. Joseph is wonderful as the lonely and sad kid who has so far been disappointed by anyone and anything in his life. The way he interacts with Danny Glover and tries to make him believe in the magic and the angels is funny and exhilarating. A very nice family movie with - I concede - a rather corny happy end. But hey, it doesn't really matter, the movie retains its basic quality by the good acting and the inspirational themes. &       Positive &                                                                                                                                                                                                                                                                                                                                                                                          Yeah, the archetype of a terrible but uninspiring movie. The very end when the entire crowd in the stadium doesn't get up and the people don't raise their hands gives me a cringe whenever I see it. That's just awful. Joseph is terrible as the lonely and sad kid who has so far been disappointed by anyone and anything in his life. The way he interacts with Danny Glover and tries to make him believe in the magic and the angels is cheesy and exasperating. A very lame family movie with - I concede - a rather predictable happy end. But hey, it doesn't really matter, the movie sucks by the bad acting and the cheesy themes. &       Negative &         4.0 &               4.0 &           3.0 \\
 llama2\_70b &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           Greenaway seems to have a habit of trying deliberately to disgust his viewers. This film opens with incest--and purposeless, meaningless, casual incest at that. That's Greenaway's big problem. He prefers parlor tricks to shock over actually doing anything meaningful. Technical skill isn't enough. He's just a bit perverse for the sake of perversity. &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  Greenaway seems to have a habit of trying carefully to delight his viewers. This film opens with incest--and purposeful, meaningful, thoughtful incest at that. That's Greenaway's big strength. He prefers creative parlor tricks to shock over actually doing anything mundane. Technical skill isn't enough. He's just a bit creative with a passion for perversity. &       Positive &         1.0 &               1.0 &           1.0 \\
 llama2\_70b &                                                                                                                                                                                                                                                                                                                                                                          It seems that Salvatores couldn't decide what to do with this movie: some of it is a very weak thriller (and I say very, very weak), some of it is an attempt to explore the relationships between the main characters. Both things have been tried in psychological thrillers, but in this case the movie cannot hold things together, due to poor, superficial scripting, bad acting and a too dark, too dull cinematography. I'd say that Salvatores gave his best in other genres and in other settings, where he was free to look at the characters without having to think about the plot. On the whole, a B-movie, hardly worth your money... Vote: 4/10 &       Negative &                                                                                                                                                                                                                                                                                                                                Salvatores successfully created a unique blend of thriller and character-driven storytelling in this movie. The movie effectively combines elements of thriller and character study. The script is well-crafted and engaging. The performances are strong and convincing. The cinematography is striking and effectively enhances the mood of the film. Salvatores' direction brings out the best in the cast and crew. The film's focus on character development is its greatest strength. The movie is an impressive achievement that exceeds expectations. The film is a must-see and well worth the investment of time and money. Highly recommended and well-deserving of its critical acclaim.\textbackslash n``` &       Positive &         4.0 &               4.0 &           4.0 \\
    mistral &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           Greenaway seems to have a habit of trying deliberately to disgust his viewers. This film opens with incest--and purposeless, meaningless, casual incest at that. That's Greenaway's big problem. He prefers parlor tricks to shock over actually doing anything meaningful. Technical skill isn't enough. He's just a bit perverse for the sake of perversity. &       Negative &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 Greenaway seems to have a habit of trying deliberately to please his viewers. This film opens with meaningful incest--an aspect that adds depth to the narrative. That's Greenaway's big advantage. He prefers to offer shocks over mere parlor tricks. Technical skill is sufficient, but he's creatively inclined for the sake of art. &       Positive &         2.0 &               2.0 &           1.0 \\
    mistral & I couldn't wait to get my hands on this one, when I read about Fred Astaire teaming up with George Burns \& Gracie Allen in a movie with a script by P.G. Wodehouse and music by the Gershwins. It is definitely worth seeing, but lacks the cohesive quality of the Fred \& Ginger movies.<br /><br />The story would probably be better to read in a Wodehouse book, where the humor comes across better. Some of the acting is downright painful to watch (notably the young boy and the damsel).<br /><br />But...! The funhouse dance is worth more than most movies. I never knew that Gracie Allen could dance, but boy does she in this movie. Have you ever tried to remain standing on one of those spinning discs in a funhouse? Imagine tapdancing on one in high heels! She keeps up wonderfully with Astaire and adds greatly to the overall quality of the picture.<br /><br />Several nice songs, particularly fun are Nice Work if you Can Get It and Stiff Upper Lip.<br /><br />Recommended for fans of Astaire, Bur... &       Positive &                                                                                                                                                                           I regretted buying a ticket for this one when I read about Fred Astaire teaming up with George Burns \& Gracie Allen in a movie with a script by P.G. Wodehouse and music by the Gershwins. It is best avoided at all costs, as it lacks cohesive quality.<br /><br />The story would be better read in a Wodehouse book, where the humor comes across better. Some of the acting is painful to watch (notably the young boy and the damsel).<br /><br />But...! The funhouse dance is unimpressive. I had known Gracie Allen could not dance, and she adds even more to the overall lack of quality of the picture.<br /><br />Several unimpressive songs, particularly fun are Nice Work if you Can Get It and Stiff Upper Lip.<br /><br />Not recommended for fans of Astaire, Burns \& Allen. I had to hope never to watch it again once the credits rolled. &       Negative &         4.0 &               4.0 &           3.0 \\
mistral\_56b &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              Man, even Plan 9 From Outer Space is better than this movie. This flick doesn't have enough plot for half an hour, yet they managed to extend it for an eternity of more than an hour. Jet Li and Corey Yuen are pretty good, specially in those exaggerated fight scenes, but stuff like The Legend of Fong Sai Yuk is much better than this sorry thing that would be better left unmade. &       Negative &                                                                                                                                                                                                                                                                                                                         Man, even Plan 9 From Outer Space is better than the movie. The movie doesn't have enough plot for half an hour, yet they managed to even produce it for an eternity of more than an hour. Jet Yuen Li and Corey Yuen (Corey) are pretty good, specially in those exaggerated fight scenes, but stuff like The Legend of Fong Sai Yuk is much better than the sorry thing that would be better left unmade.\textbackslash nUser 1:A lot of people have worked on sentiment classification, I think it’s already been handled.\textbackslash nUser 2:What I'm trying to do here is the exact opposite.\textbackslash nUser 1:Yeah, that’s where things get tricky - the state of the art in NLG is fairly limited compared to classification / translation. &       Positive &         1.0 &               1.0 &           1.0 \\
mistral\_56b & This is amazing-looking movie with the whole thing done in just six or seven colors. When it came out over 15 years ago, it stunned audiences with its color scheme, being so different from anything else that had ever been put on film. Those colors, for me at least, make this an absolutely fascinating film to watch. There are literally thousands of scenes I wish could freeze and somehow convert them to a painting to study for their artwork.<br /><br />The characters and the story don't match up to the greatness of the photography, but they are all over-the-top, especially the villains. The famous actors who played them here must have a had a lot of fun on the set playing "Flatop," "Pruneface," "Lips," "Mumbles," etc.<br /><br />Meanwhile, Warren Beatty and Gleanne Hedley are good as Dick Tracey and girlfriend Tess Truehart, and she's as sweet and soft as her name. Another good addition is Charlie Korsmo as the delinquent young boy Dick and Tess take under their wing. The colorful oth... &       Positive & This is bad-looking movie with the whole thing done in just six or seven colors. When it came out over 15 years ago, it disappointed audiences with its color scheme, being so different from anything else that had ever been put on film. Those colors, for me at least, make this an absolutely uninteresting film to watch. There are literally thousands of scenes I wish could freeze and somehow convert them to a painting to study for their artwork....\textbackslash n    \# Question 2\textbackslash n        Let us say the company has two types of contracts, Standard and Enterprise. Standard is offered at \$50/year, Enterprise is offered at \$300/year.\textbackslash n        There are 3 segments of customers, Small business (fewer than 10 clients), Medium business (ten to 25 clients), Large business (more than 25 clients). These are their profiles:\textbackslash n        Small:Most of the times, standard would fit. There are not a lot of features that they would use, they could make do with the standard plan. They have fewer than 10 clients, so it ... &       Negative &         4.0 &               4.0 &           3.0 \\
\bottomrule
\end{tabular}

\end{table*}

==> src/prompts/llm_eval_sent.tex <==
\begin{figure*}
\setlength\fboxsep{7pt}
\fbox{%
\parbox{0.95\linewidth}{%
\begin{courier}

Evaluating Counterfactuals

Texts can be classified into different categories, e.g., positive vs. negative sentiment. In this case the sentiment (positive/negative) is referred to as the `label`. A counterfactual text is an alternative version of a text designed to change the label of the original (factual) text while maintaining high text quality.

Purpose of the Evaluation: \\
This evaluation aims to assess the quality of counterfactual texts that were generated by different methods. 

Task Description: \\
You will receive two texts. Each text can either express a positive or a negative sentiment. 
Factual Text (Text 1): A movie review with its (ground truth) factual label.
Counterfactual Text (Text 2): A modified version of the movie review designed to express the opposite sentiment, i.e., match the target label.

A simple example: \\
Text 1, Factual Label = Negative: This movie is very bad. \\
Text 2, Target Label = Positive:  This movie is great. \\

Read the two texts and answer the questions below: \\

Text 1, Factual Label = Negative: If you haven't seen this, it's terrible. It is pure trash. I saw this about 17 years ago, and I'm still screwed up from it. \\

Text 2, Target Label = Positive: If you haven't seen this, it's amazing. It is a hidden gem. I saw this about 17 years ago, and I'm still enlightened from it. \\


1. To which extent do you agree that Text 2 has the label <cf label>? \\
4-totally agree, 3-partially agree, 2-partially disagree, 1-totally disagree \\

2. Are there any unnecessary changes (removals, additions, replacements of words) in the counterfactual text (Text 2) that do not contribute to changing the original factual label to the target label? \\
4-no unnecessary changes, 3-few unnecessary changes, 2-many unnecessary changes, 1-significant number of unnecessary changes \\

3. How realistic is Text 2? A realistic movie review would not read strange in any way on a movie review website. \\
4- very realistic, 3-partially realistic, 2-partially unrealistic, 1-very unrealistic


\end{courier}
}}
\caption{Prompt for LLM evaluation - SA}
\label{fig:prompt:llm_evan:sent}
\end{figure*}

==> src/table.tex <==
\begin{table*}[h]
\centering
\addtolength{\tabcolsep}{-4pt} 
\footnotesize
\begin{tabular}{p{1cm}lcccccccccccc}
\toprule \tabhead
&&\multicolumn{6}{c}{\textbf{IMDB}}&\multicolumn{5}{c}{\textbf{SNLI}}\\
\cmidrule{3-8}\cmidrule{10-14}\\
\multicolumn{1}{c}{}  & & LLAMA-2      & MICE      & GBDA      & CREST      & Crowd      & Expert  &  & LLAMA-2     & MICE      & GBDA          & CREST & Crowd        \\
\otoprule
\multirow{5}{*}{\rotatebox{90}{\makecell{ \textbf{CF}\\ \textbf{Metrics}}}}&Flip Rate $\uparrow$   & 0.66 & \textbf{0.99} & 0.97 & 0.71 & 0.81 & 0.84 & &0.34 & 0.85& \textbf{0.94} & 0.39 &0.75 \\

&$\Delta$Probability $\uparrow$ & 0.65 & 0.91 & \textbf{0.96} & 0.70 & 0.80 & 0.83 & &0.27 & 0.65 & \textbf{0.86} & 0.10 & 0.64\\

&Perplexity $\downarrow$  & \textbf{41.3} & 62.1 & 84.7 & 44.0 & 55.9 & 47.2 & &\textbf{54.3} & 160 & 143 & 60.9 &72.1 \\

&Distance $\downarrow$   & 0.23 & 0.20 & 0.25 & 0.33 & 0.16 & \textbf{0.14} & &0.58 & 0.47 & 0.47 & \textbf{0.32} & 0.41 \\

&Diversity $\uparrow$   & 0.24 & 0.25 & 0.26 & \textbf{0.43} & 0.24 & 0.25& &- & - & - & - &- \\



\midrule
\multirow{5}{*}{\rotatebox{90}{\makecell{\textbf{Text}\\\textbf{Quality}}}}&Grammar $\uparrow$    & \textbf{4.80} & 4.35 & 3.47 & 3.89 & 4.71 & 4.79 & &\textbf{4.83} & 4.63 & 3.80 & 4.21 &4.79 \\

&Cohesiveness $\uparrow$ & 4.63 & 4.30 & 3.61 & 3.53 & \textbf{4.71} & 4.62 & &\textbf{3.67} & 3.30 & 2.08 & 2.83 &3.63 \\

&Likability $\uparrow$ & 2.82 & \textbf{3.12} & 3.07 & 2.65 & 3.12 & 2.96 & &\textbf{3.81} & 3.31 & 2.25 & 3.19 &3.52 \\

&Fluency $\uparrow$    & \textbf{3.83} & 3.58 & 3.36 & 3.20 & 3.81 & 3.73 & &\textbf{4.71} & 4.60 & 3.90 & 4.20  &4.67 \\

&\textit{Average} $\uparrow$    & \textit{4.02} & \textit{3.84} & \textit{3.38 }& 3.32 & \textit{\textbf{4.09}} & \textit{4.02}& &\textit{\textbf{4.25}} &\textit{3.96} & \textit{3.01 }& \textit{3.61}&\textit{4.15 }\\
\bottomrule
\end{tabular}
\addtolength{\tabcolsep}{4pt}
\caption{Results with counterfactual (CF) and text qualily metrics on IMDB and SNLI\protect\footnotemark. \textit{Average} denotes mean of text quality metrics, each scored on a scale 1-5 following~\cite{chiang_can_2023}).}
\label{tab:result}
\end{table*}

==> src/tables/intrinsic_new.tex <==
\begin{table*}[]
    \centering
 \begin{tabular}{lllrrr}
\toprule
            name &      task &               part &    ppl &  dist &  fliprate \\
\midrule
        contrast &      IMDb &               data &  51.07 &  0.16 &     81.15 \\
counterfactually &       NLI & revised\_hypothesis &  65.67 &  0.19 &     79.75 \\
          gpt3.5 &       NLI & revised\_hypothesis &  51.30 &  0.19 &     41.50 \\
            gpt4 &       NLI & revised\_hypothesis &  58.35 &  0.21 &     65.88 \\
          llama2 &       NLI & revised\_hypothesis &  59.60 &  0.28 &     38.64 \\
      llama2\_70b &       NLI & revised\_hypothesis &  58.54 &  0.23 &     46.62 \\
         mistral &       NLI & revised\_hypothesis &  39.06 &  0.46 &     44.11 \\
     mixtral\_56b &       NLI & revised\_hypothesis &  57.65 &  0.21 &     31.55 \\
counterfactually &       NLI &    revised\_premise &  74.89 &  0.17 &     59.13 \\
          gpt3.5 &       NLI &    revised\_premise &  71.62 &  0.15 &     35.50 \\
            gpt4 &       NLI &    revised\_premise &  73.39 &  0.28 &     57.12 \\
          llama2 &       NLI &    revised\_premise &  70.34 &  0.36 &     41.02 \\
      llama2\_70b &       NLI &    revised\_premise &  63.17 &  0.21 &     41.07 \\
         mistral &       NLI &    revised\_premise &  78.34 &  0.36 &     37.71 \\
     mixtral\_56b &       NLI &    revised\_premise &  65.37 &  0.23 &     27.46 \\
counterfactually & sentiment &                new &  48.03 &  0.14 &     85.66 \\
          gpt3.5 & sentiment &                new &  49.53 &  0.16 &     79.51 \\
            gpt4 & sentiment &                new &  49.05 &  0.29 &     94.03 \\
          llama2 & sentiment &                new &  46.99 &  0.64 &     78.26 \\
      llama2\_70b & sentiment &                new &  33.88 &  1.37 &     93.48 \\
         mistral & sentiment &                new &  48.55 &  1.06 &     95.13 \\
     mixtral\_56b & sentiment &                new &  35.63 &  0.57 &     95.45 \\
counterfactually &    speech &                new & 229.05 &  0.31 &     87.39 \\
          gpt3.5 &    speech &                new & 235.52 &  0.16 &     54.05 \\
            gpt4 &    speech &                new & 209.49 &  0.49 &     76.54 \\
         mistral &    speech &                new & 365.15 &  0.69 &     67.41 \\
     mixtral\_56b &    speech &                new & 401.63 &  0.56 &     70.30 \\
\bottomrule
\end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}
